ParTEETor: A System for Partial Deployments of TEEs within Tor

The Tor anonymity network allows users such as political activists and those under repressive governments to protect their privacy when communicating over the internet. At the same time, Tor has been demonstrated to be vulnerable to several classes of deanonymizing attacks that expose user behavior and identities. Prior work has shown that these threats can be mitigated by leveraging trusted execution environments (TEEs). However, previous proposals assume that all relays in the network will be TEE-based-which as a practical matter is unrealistic. In this work, we introduce ParTEETor, a Tor-variant system, which leverages partial deployments of TEEs to thwart known attacks. We study two modes of operation: non-policy and policy. Non-policy mode uses the existing Tor relay selection algorithm to provide users incident security. Policy mode extends the relay selection algorithm to address the classes of attacks by enforcing a specific TEE circuit configuration. We evaluate ParTEETor for security, performance, and privacy. Our evaluation demonstrates that at even a small TEE penetration (e.g., 10% of relays are TEE-based), users can reach performance of Tor today while enforcing a security policy to guarantee protection from at least two classes of attacks. Overall, we find that partial deployments of TEEs can substantially improve the security of Tor, without a significant impact on performance or privacy.

==> conf-format/08.relatedwork.tex <==

\section{Related Work}

%\tbd{ - Can be trimmed}
\begin{comment}
\shortsection{TEE-based Applications}
As the effort of integrating applications with TEEs is generally nontrivial, recent works have been published allowing for easier integration. One approach to simplifying the porting of applications is by using Library OSes. Essentially, all core functions of an operating system (e.g., network functions) are placed within a module running in a TEE, increasing the size of the TCB (trusted computing base) but allowing for unmodified code to reap the security benefits of TEEs with minimal modification. 
Haven~\cite{haven} was one of the first library OSes to leverage TEEs in cloud computing.
Panoply~\cite{panoply} presented a smaller TCB compared to Haven, while still allowing for applications to run within micro-containers which abstract the OS functionality.  
Graphene-SGX~\cite{graphene}, motivated by the critiques of library OSes, presented a practical TEE system with performance exceeding both Haven and Panoply. 
These works all present systems which provide for easy portability of applications into TEEs. Our work presents how the security guarantees of TEEs can be leveraged to improve the security of the Tor network. 

\end{comment}

% \shortsection{Securing Tor with TEEs}
%microsoft.com/en-us/research/uploads/prod/2019/03/panoply_ndss17.pdf
%https://taesoo.kim/pubs/2016/jain:opensgx.pdf
%https://dl.acm.org/doi/10.1145/2834050.2834100
A few notable works have explored the union of TEEs and the Tor network in various ways. 
Panoply~\cite{panoply}, the library OS for integrating applications with TEEs, presents a case study on Tor. 
Shinde \textit{et al.} integrate all Tor Directory Authority protocol into their system in order to prevent adversaries from manipulating the consensus of the network to allows malicious relays to be accepted. 
Jain \textit{et al.} present OpenSGX~\cite{opensgx}, a system that emulates SGX at an instruction level. In their evaluation, they are motivated in preventing attacks that exploit the private keys of directory authorities and exit nodes, in which they integrate the 
cryptographic functions of the Tor protocol into their system.  Specifically, all identity key generation and storage for directory authorities, as well as exit relays, is moved into the TEE. Additionally, the onion key of the exit node and the consensus documents are stored in the TEE. 
These works look at increasing the security of select Tor components, while our work analyzes how the specific position of TEEs in a Tor circuit can mitigate attacks.

\begin{comment}
\shortsection{Attacks on Tor}
% The Tor protocol's threat model aims to prevent traffic analysis attacks~\cite{tor2004original}, which are used to identify points in the network to attack by observing patterns in traffic. Tor does not, however, protect against traffic confirmation attacks, which involve adversaries viewing both the entry and exit points of the network in order to correlate sender and receiver.
%Tor is still vulnerable to many traffic confirmation attacks, in addition to some traffic analysis attacks, as have been revealed for years since Tor's inception. In general, the adversarial goal for these attacks is to deanonymize users. 
Attacks on the Tor network and its users are constantly being revealed each year. Attacks targeting the network itself include DoS such as the Sniper attack~\cite{jansen_sniper_2014} which floods circuits with \textit{sendme} cells, and the CellFlood attack~\cite{cellflood}, which floods circuits with \textit{create} cells. Sybil attacks~\cite{sybil} admit a large number of malicious relays at once. As these attacks are not deanonymizing attacks, we do not consider these in our work. 
\sloppy Attacks that are leveraged by the Tor client~\cite{murdoch_hot_2006, clockskew} use the clock skew of the client's computer to deanonymize hidden services. We do not consider these attacks, as they are outside of our threat model, with the client being malicious. 
Our work focuses on specific classes of deanonymizing attacks where malicious relays exploit circuit details such as circuit IDs and stream IDs.
\end{comment}

% survey paper where these attacks came from: 
%https://arxiv.org/pdf/2009.13018.pdf#page=25&zoom=100,65,756


% \subsection{Modified Tor Relay Selection Algorithms}
% There have been many published works on the Tor relay selection algorithm and proposed improvements to it. Wang \textit{et al.} propose a latency biased algorithm~\cite{node_latency_alg}, in which the congestion of Tor relays is calculated and added as a property. Then, when selecting relays for a circuit, a subset of all potential relays is chosen, and the relay with the least congestion is then chosen from there. This is done for each relay in the circuit. 
% Imani \textit{et al.} propose a geographic-aware algorithm~\cite{geo_bw_alg} which adds an additional weight to relays that takes into account their geographic location. In addition to the weight of the bandwidth, this geographic weight allows for relays with shorter distances from each other to be more likely to be chosen, improving the performance of circuits. 
% Snader \textit{et al.}'s algorithm~\cite{tuneup_alg} and Zhang \textit{et al.}'s algorithm \cite{client_bias_alg} take in an additional parameter from the client denoting their desired performance vs anonymity. This parameter is then multiplied by a random variable, then relays are chosen with this additional weight added to them. Both works found that allowing users to specify their performance or anonymity expectations results in little to no performance degradation and meets users preferences. 
% Kiran \textit{et al.} present a selection strategy that is similar to the previous two algorithms in that it takes in a parameter from the client on their expected performance~\cite{bucket_alg}. The relays are separated into two categories based on their bandwidth allowance, and with the client input, potential relays to be chosen for a circuit are based on which category it falls into. 

%\cite{adversary_selection_alg} - can go over this too if needed






